Egoshots, an ego-vision life-logging dataset and semantic fidelity metric to evaluate diversity in image captioning models

Image captioning models have been able to generate grammatically correct and human understandable sentences. However most of the captions convey limited information as the model used is trained on datasets that do not caption all possible objects existing in everyday life. Due to this lack of prior information most of the captions are biased to only a few objects present in the scene, hence limiting their usage in daily life. In this paper, we attempt to show the biased nature of the currently existing image captioning models and present a new image captioning dataset, Egoshots, consisting of 978 real life images with no captions. We further exploit the state of the art pre-trained image captioning and object recognition networks to annotate our images and show the limitations of existing works. Furthermore, in order to evaluate the quality of the generated captions, we propose a new image captioning metric, object based Semantic Fidelity (SF). Existing image captioning metrics can evaluate a caption only in the presence of their corresponding annotations; however, SF allows evaluating captions generated for images without annotations, making it highly useful for real life generated captions.

==> ToDo.tex <==
Image captioning:
https://github.com/jiasenlu/NeuralBabyTalk
@article{DBLP:journals/corr/abs-1803-09845,
  author    = {Jiasen Lu and
               Jianwei Yang and
               Dhruv Batra and
               Devi Parikh},
  title     = {Neural Baby Talk},
  journal   = {CoRR},
  volume    = {abs/1803.09845},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.09845},
  archivePrefix = {arXiv},
  eprint    = {1803.09845},
  timestamp = {Mon, 13 Aug 2018 16:46:14 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1803-09845.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@ARTICLE{Li20,
       author = {{Li}, Junnan and {Xiong}, Caiming and {Socher}, Richard and
         {Hoi}, Steven},
        title = "{Towards Noise-resistant Object Detection with Noisy Annotations}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Computer Vision and Pattern Recognition},
         year = 2020,
        month = mar,
          eid = {arXiv:2003.01285},
        pages = {arXiv:2003.01285},
archivePrefix = {arXiv},
       eprint = {2003.01285},
 primaryClass = {cs.CV},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200301285L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@InProceedings{Lu_2017_CVPR,
author = {Lu, Jiasen and Xiong, Caiming and Parikh, Devi and Socher, Richard},
title = {Knowing When to Look: Adaptive Attention via a Visual Sentinel for Image Captioning},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}
-> abs: Attention-based neural encoder-decoder frameworks have been widely adopted for image captioning. Most methods force visual attention to be active for every generated word. However, the decoder likely requires little to no visual information from the image to predict non-visual words such as “the” and “of”. Other words that may seem visual can often be predicted reliably just from the language model e.g., “sign” after “behind a red stop” or “phone” following “talking on a cell”. In this paper, we propose a novel adaptive attention model with a visual sentinel. At each time step, our model decides whether to attend to the image (and if so, to which regions) or to the visual sentinel. The model decides whether to attend to the image and where, in order to extract meaningful information for sequential word generation. We test our method on the COCO image captioning 2015 challenge dataset and Flickr30K. Our approach sets the new state-of-the-art by a significant margin

Context-Aware Captions From Context-Agnostic Supervision Ramakrishna Vedantam, Samy Bengio, Kevin Murphy, Devi Parikh, Gal Chechik; The IEEE Conference on Computer Vision and Pattern Recognition (CVPR), 2017, pp. 251-260
@InProceedings{Vedantam_2017_CVPR,
author = {Vedantam, Ramakrishna and Bengio, Samy and Murphy, Kevin and Parikh, Devi and Chechik, Gal},
title = {Context-Aware Captions From Context-Agnostic Supervision},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
}
Abstract 

We introduce an inference technique to produce discriminative context-aware image captions (captions that describe differences between images or visual concepts) using only generic context-agnostic training data (captions that describe a concept or an image in isolation). For example, given images and captions of "siamese cat" and "tiger cat", we generate language that describes the "siamese cat" in a way that distinguishes it from "tiger cat". Our key novelty is that we show how to do joint inference over a language model that is context-agnostic and a listener which distinguishes closely-related concepts. We first apply our technique to a justification task, namely to describe why an image contains a particular fine-grained category as opposed to another closely-related category of the CUB- 200-2011 dataset. We then study discriminative image captioning to generate language that uniquely refers to one of two semantically-similar images in the COCO dataset. Evaluations with discriminative ground truth for justification and human studies for discriminative image captioning reveal that our approach outperforms baseline generative and speaker-listener approaches for discrimination.

Taking a HINT: Leveraging Explanations to Make Vision and Language Models More Grounded Ramprasaath R. Selvaraju, Stefan Lee, Yilin Shen, Hongxia Jin, Shalini Ghosh, Larry Heck, Dhruv Batra, Devi Parikh; The IEEE International Conference on Computer Vision (ICCV), 2019, pp. 2591-2600

Abstract 

Many vision and language models suffer from poor visual grounding -- often falling back on easy-to-learn language priors rather than basing their decisions on visual concepts in the image. In this work, we propose a generic approach called Human Importance-aware Network Tuning (HINT) that effectively leverages human demonstrations to improve visual grounding. HINT encourages deep networks to be sensitive to the same input regions as humans. Our approach optimizes the alignment between human attention maps and gradient-based network importances -- ensuring that models learn not just to look at but rather rely on visual concepts that humans found relevant for a task when making predictions. We apply HINT to Visual Question Answering and Image Captioning tasks, outperforming top approaches on splits that penalize over-reliance on language priors (VQA-CP and robust captioning) using human attention demonstrations for just 6% of the training data.
@InProceedings{Selvaraju_2019_ICCV,
author = {Selvaraju, Ramprasaath R. and Lee, Stefan and Shen, Yilin and Jin, Hongxia and Ghosh, Shalini and Heck, Larry and Batra, Dhruv and Parikh, Devi},
title = {Taking a HINT: Leveraging Explanations to Make Vision and Language Models More Grounded},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}





% security copy
% DO NOT TOUCH HERE UNLESS MAKING COPY BEFORE, THE MARGINS ARE NOT PRESERVED FRO SOME REASON (THIS IS BEST WAY I COULD FIND TO ALING ALEJANDRO AND MY NAME TO KEEP BALANCED LAYOUT
\author{Pranav Agarwal \\
INRIA RITS, Paris, France\\
\texttt{pranav2109@hotmail.com}\\
\And % same line
 Alejandro Betancourt\\
 LANDING AI, Colombia %Eindhoven University of Technology, Netherlands\\
 \texttt{abetan16@gmail.com}\\
\AND   % IMPORTANT FOR  NEW LINE (ALL CAPITAL)  %And makes the name in bold
Vana Panagiotou*\\
Signal Ocean, Greece. \\% Philips Research\\
\texttt{panagiotou.vana@gmail.com}\\
\And
Natalia ~Díaz-Rodríguez\thanks{Work partially done during Díaz-Rodríguez and Panagiotou' internships at Philips Research, and Betancourt' stay at Eindhoven University of Technology, Netherlands.} \\
U2IS, ENSTA, Institut Polytechnique Paris and\\
INRIA Flowers, France\\
\texttt{natalia.diaz@ensta-paris.fr}\\
%   \And
%   Coauthor \\
%   Affiliation \\
%   Address \\
%   \texttt{email} \\
}
